Mass Variance from Archival X-ray Properties of Dark Energy Survey Year-1 Galaxy Clusters

Using archival X-ray observations and a log-normal population model, we estimate constraints on the intrinsic scatter in halo mass at fixed optical richness for a galaxy cluster sample identified in Dark Energy Survey Year-One (DES-Y1) data with the redMaPPer algorithm. We examine the scaling behavior of X-ray temperatures, $T_X$, with optical richness, $\lambda_{RM}$, for clusters in the redshift range $0.2<z<0.7$. X-ray temperatures are obtained from Chandra and XMM observations for 58 and 110 redMaPPer systems, respectively. Despite non-uniform sky coverage, the $T_X$ measurements are $> 50\%$ complete for clusters with $\lambda_{RM} > 130$. Regression analysis on the two samples produces consistent posterior scaling parameters, from which we derive a combined constraint on the residual scatter, $\sigma_{\ln Tx | \lambda} = 0.275 \pm 0.019$. Joined with constraints for $T_X$ scaling with halo mass from the Weighing the Giants program and richness--temperature covariance estimates from the LoCuSS sample, we derive the richness-conditioned scatter in mass, $\sigma_{\ln M | \lambda} = 0.30 \pm 0.04\, _{({\rm stat})} \pm 0.09\, _{({\rm sys})}$, at an optical richness of approximately 70. Uncertainties in external parameters, particularly the slope and variance of the $T_X$--mass relation and the covariance of $T_X$ and $\lambda_{RM}$ at fixed mass, dominate the systematic error. The $95\%$ confidence region from joint sample analysis is relatively broad, $\sigma_{\ln M | \lambda} \in [0.14, \, 0.55]$, or a factor ten in variance.

==> DES X-ray scaling of redMaPPer clusters (arXiv submission)/newcommands.tex <==
\newcommand{\wtg}{WtG}
\newcommand{\clash}{CLASH}
\newcommand{\cccp}{CCCP}
\newcommand{\locuss}{LoCuSS}

\newcommand{\simname}{\texttt{FOX}}
\newcommand{\rockstar}{{\tt Rockstar}}
\newcommand{\mangle}{\texttt{mangle}}

\newcommand{\gmag}{$g$}
\newcommand{\rmag}{$r$}
\newcommand{\imag}{$i$}
\newcommand{\zmag}{$z$}
\newcommand{\griz}{$g,r,i,z$}
\newcommand{\umg}{$u-g$}
\newcommand{\gmr}{$g-r$}
\newcommand{\rmi}{$r-i$}
\newcommand{\imz}{$i-z$}

\newcommand{\psfmag}{\texttt{psfmag}}
\newcommand{\modelmag}{\texttt{modelmag}}
\newcommand{\cmodelmag}{\texttt{cmodelmag}}

\newcommand{\radec}{$\alpha,\delta$}

\newcommand{\devauc}{De Vaucouleurs'}

\newcommand{\gammat}{\mbox{$\gamma^{\intercal}$}}

% peter's versions
\newcommand{\pzs}{\mbox{$p_\mathrm{phot}(z_{\mathrm{s},i})$ }}
\newcommand{\zsi}{\mbox{$z_{\mathrm{s},i}$}}
\newcommand{\zlj}{\mbox{$z_{\mathrm{l},j}$}}
\newcommand{\etan}{\mbox{$e^{\intercal}$}}
\newcommand{\etanij}{\mbox{$e^{\intercal}_{j,i}$}}

% erin's versions
%\newcommand{\pzs}{\mbox{$p(z_{\mathrm{s},i})$ }}
%\newcommand{\pzs}{\mbox{$p(z^i_{\mathrm{s}})$ }}
%\newcommand{\zsi}{\mbox{$z^i_\mathrm{s}$}}
%\newcommand{\zlj}{\mbox{$z^i_\mathrm{l}$}}
%\newcommand{\etani}{\mbox{$e^i_\mathrm{t}$}}

\newcommand{\gammacross}{$\gamma_\times$}
\newcommand{\deltasig}{$\Delta \Sigma$}
\newcommand{\dsig}{$\Delta\Sigma$}
\newcommand{\dsigr}{$\Delta\Sigma(R)$}
\newcommand{\dsigmis}{$\Delta\Sigma_{\mathrm{mis}}$}
\newcommand{\deltaplus}{$\Delta \Sigma_+$}
\newcommand{\deltacross}{$\Delta \Sigma_\times$}
\newcommand{\deltarho}{$\Delta \rho$}
\newcommand{\movr}{$M(<r)$}
\newcommand{\sigmacrit}{$\Sigma_{\mathrm{crit}}$}
\newcommand{\scinv}{$\Sigma^{-1}_{\mathrm{crit}}$}
\newcommand{\hinv}{h^{-1}}


\newcommand{\photoz}{\mbox{photo-$z$}}
\newcommand{\photozs}{\mbox{photo-$z$s}}

\newcommand{\lenszmax}{0.8}
\newcommand{\lenszmin}{0.2}

\newcommand{\hrs}{$^{\mathrm h}$}
\newcommand{\minutes}{$^{\mathrm m}$}

\newcommand{\redmapper}{redMaPPer}
\newcommand{\rmversion}{6.3.3}
\newcommand{\ngmix}{\textsc{ngmix}\ }

\newcommand{\annz}{\textsc{annz2}}
\newcommand{\skynet}{\textsc{skynet}}
\newcommand{\tpz}{\textsc{tpz}}
\newcommand{\bpz}{\textsc{bpz}}
\newcommand{\balrog}{\textsc{Balrog}}
\newcommand{\cosmosis}{\textsc{CosmoSIS}}

\newcommand{\neffngmix}{5.7}
\newcommand{\ngmixlowzbiasneg}{$-0.04$}
\newcommand{\recommendedprior}{0.05}
\newcommand{\njack}{40}
\newcommand{\shapenoise}{0.22}
\newcommand{\rmax}{30}
\newcommand{\imshape}{{\textsc{im3shape}}}
\newcommand{\snr}{S/N}
\newcommand{\metacal}{\textsc{metacalibration}\ }

\newcommand{\msun}{\mathrm{M}_{\odot}}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\brown}[1]{\textcolor{brown}{#1}}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}


\newcommand{\edens}{$e_q$}
\newcommand{\lfsens}{\mbox{\boldmath $s$}}

\newcommand\avg[1]{\langle #1 \rangle}
\newcommand{\Scrit}{\Sigma_{\rm crit}}
\newcommand{\Mpc}{\mathrm{Mpc}}
\newcommand{\hMpc}{h^{-1}\ \Mpc}

\newcommand{\fcl}{f_\mathrm{cl}}

\newcommand{\Mobs}{M_{\rm obs}}
\newcommand{\Mtrue}{M_{\rm true}}
\newcommand{\Mwl}{M_{\rm wl}}
\newcommand{\Var}{{\rm Var}}

\newcommand{\lnM}{{\rm ln}M}
\newcommand{\MF}{\frac{dn(M,z)}{d\, \ln M}}
\newcommand{\MFmu}{\frac{dn(\mu,z)}{d\mu}}
\newcommand{\varmassfullone}{\sigma_{\mu | s}^2}
\newcommand{\sigmamu}{\sigma_{\mu | s}}
\newcommand{\lamRM}{\lambda_{\rm RM}}

\newcommand{\chandra}{\emph{Chandra}}
\newcommand{\xmm}{\emph{XMM}}
\newcommand{\RM}{redMaPPer}

\newcommand{\Rmis}{R_{\rm mis}}
\newcommand{\fmis}{f_{\rm mis}}
\newcommand{\cmis}{c_{\rm mis}}

\newcommand{\Am}{A_{\rm m}}

\newcommand{\lkhd}{{\cal L}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calC}{{\cal C}}




